Learning Where to Look: Data-Driven Viewpoint Set Selection for 3D Scenes

The use of rendered images, whether from completely synthetic datasets or from 3D reconstructions, is increasingly prevalent in vision tasks. However, little attention has been given to how the selection of viewpoints affects the performance of rendered training sets. In this paper, we propose a data-driven approach to view set selection. Given a set of example images, we extract statistics describing their contents and generate a set of views matching the distribution of those statistics. Motivated by semantic segmentation tasks, we model the spatial distribution of each semantic object category within an image view volume. We provide a search algorithm that generates a sampling of likely candidate views according to the example distribution, and a set selection algorithm that chooses a subset of the candidates that jointly cover the example distribution. Results of experiments with these algorithms on SUNCG indicate that they are indeed able to produce view distributions similar to an example set from NYUDv2 according to the earth mover's distance. Furthermore, the selected views improve performance on semantic segmentation compared to alternative view selection algorithms.

==> viewpoint.tex <==
% !TeX root = hcv.tex
\section{\todo{Viewpoint Selection}}

\todo{Describe problem of viewpoint selection including: viewpoint parameterization, generating candidate cameras, scoring viewpoints, finding a set of k camera.}

\paragraph{Viewpoint parameterization.}
A viewpoint is parameterized according to the following six degrees of freedom: $(x,y,z,n_\theta,n_\phi, \theta)$. These comprise a 3D position, the polar and azimuthal angles of the normal vector to the viewpoint plane, and the rotation around the normal vector. Field of view and aspect ratio of the viewpoint are considered fixed as a part of the input constraints: the output viewpoint may need to adhere to such constraints during training. Viewpoint roll is included in the parameterization despite its rare use by humans, as captured images are rarely perfectly aligned but viewpoints with near-zero roll best match the object distribution data from human-captured images.

\paragraph{RGBD object distribution data.} 
Input ground truth data is assumed to take the general form that follows. Each category is associated with a set of pixels that have been tagged by a human as belonging to that category. Pixels are given as an $(x,y,d)$ tuple that specifies the image space coordinates and recorded depth value at those coordinates. This formulation does not fully exploit the information present in the NYUDv2 dataset: such data is difficult to acquire but the viewpoint selection algorithm is more broadly applicable. In particular, this formulation does not require that every pixel in an image be tagged with a category, nor that instances of a given category be separately identified. The consequences of the latter generalization eliminate much of the usefulness of simple distribution measures and justify use of the entire set of raw tagged pixels. Consider the image space centroid for a category: this measure is highly unstable for categories that have multi-modal distributions on a per-instance scope, such as cabinets. Reasoning in terms of the entire distribution sidesteps such pitfalls.


